Identity leakage through accent cues in voice anonymisation

Voice anonymisation is used to conceal voice identity while preserving linguistic content. Even if anonymisation seems strong, non-timbral cues such as accent that remain post-anonymisation can help re-identification and reveal sensitive socio-demographic traits. We report a study of residual accent information involving multiple anonymisation systems. We highlight the role of accent using speaker verification, accent verification, and accent classification using a set of embeddings focusing on timbral, non-timbral and accent-related information and show the extent to which related cues facilitate reidentification post anonymisation. Results show that, while some systems are robust to reidentification attempts using accent cues, others leave residual, speaker-dependent, accentrelated cues which can be used to reveal the voice identity. We also highlight accent-dependent variation in anonymisation performance, raising fairness concerns, and show that a system with characterlevel conditioning can help obfuscate identity-revealing accent cues, reducing accent-identification accuracy by 68% on average and improving overall anonymisation performance by 11% relative.

==> rebutall.tex <==

% Version Soft
We thank all the reviewers for their careful evaluation and largely positive feedback. With two entirely positive reviews (3308 and 6FBA), we provide detailed clarifications for the three points raised by Reviewer 5A16. While we can understand some of the comments, they mainly concern additional work that we ourselves suggest rather than weaknesses that affect the validity of our contributions.

The ablation study proposed by the reviewer is exactly what is already described in the Discussion section. The inclusion of speaker verification, accent verification and accent identification results derived from the use of multiple embedding models and a diverse set of anonymisation systems provides a robust and sufficient basis for our claims. We hence interpret this remark as a valuable suggestion for more detailed analysis, which we suggest ourselves in the paper.

Concerning speech naturalness and intelligibility, there is a misunderstanding regarding the primary scope of our study. We already wrote explicitly that utility evaluation, including naturalness and intelligibility, is an important direction for future work.  The focus of our contributions is instead upon privacy and fairness risks induced by residual accent cues. We are entirely satisfied that this is clear from the opinion supported by the other two positive reviews. As clearly stated in the Discussion, we indicate that strong accent suppression MAY reduce naturalness and intelligibility; no categorical claim is made.

We cannot disagree with the suggestion that training using accent-balanced datasets would be welcome. Of course, it would be; however, such datasets are not currently available at scale. Our experiments rely on the widely used Common Accent dataset, and the results obtained are sufficient to support our conclusions.  It is worth noting that training with accent-balanced datasets would probably improve results, not degrade them.
 

%Version Nick
% We thank all the reviewers for their careful evaluation and largely positive feedback. With two entirely positive reviews from 3308 and 6FBA, we focus only upon the one reviewer 5A16 who raised three negative points. While we can understand some of the comments, they appear not to target the specific contributions of our work or appear to be critical of us for not having done some additional work that we ourselves suggest.
 
% The ablation study proposed by the reviewer is exactly what is already described in the Discussion section. The inclusion of speaker verification, accent verification and accent identification results derived from the use of multiple embedding models and a diverse set of anonymisation systems is already perfectly sufficient to support our claims. We hence interpret this remark as merely a suggestion for more detailed analysis, which we suggest ourselves in the paper, rather than a weakness.

% The reviewer has misinterpreted our claims and also missed the point. We already wrote explicitly that utility evaluation, including naturalness and intelligibility, is an important direction for future work.  The focus of our contributions is instead upon privacy and fairness risks induced by residual accent cues. We are entirely satisfied that this is more than sufficiently clear, an opinion supported by the other two positive reviews. As stated in the Discussion, we indicate that strong accent suppression MAY reduce naturalness and intelligibility. We do not make a categorical claim. 

% We cannot disagree with the suggestion that training using accent-balanced datasets would be welcome.  Of course it would be, and we would be more understanding of this criticism if such datasets were actually available. Since they are not, the reviewer does not offer any specific suggestions, and since the results derived using the widely-used Common Accent dataset are nonetheless sufficient to support our claims, we do not accept the criticism.  In any case, training with accent-balanced datasets would probably improve results, not degrade them.
